Taking Advice from ChatGPT

A growing literature studies how humans incorporate advice from algorithms. This study examines an algorithm with millions of daily users: ChatGPT. In a preregistered study, 118 student participants answer 2,828 multiple-choice questions across 25 academic subjects. Participants receive advice from a GPT model and can update their initial responses. The advisor's identity ("AI chatbot" versus a human "expert"), presence of a written justification, and advice correctness do not significantly affect weight on advice. Instead, participants weigh advice more heavily if they (1) are unfamiliar with the topic, (2) used ChatGPT in the past, or (3) received more accurate advice previously. The last two effects -- algorithm familiarity and experience -- are stronger with an AI chatbot as the advisor. Participants that receive written justifications are able to discern correct advice and update accordingly. Student participants are miscalibrated in their judgements of ChatGPT advice accuracy; one reason is that they significantly misjudge the accuracy of ChatGPT on 11/25 topics. Participants under-weigh advice by over 50% and can score better by trusting ChatGPT more.

==> tables/topic_counts.tex <==
\begin{tabular}{lrll}
\toprule
                         Topic/Task &  Question Count &                                        description &   Familiarity Topic \\
\midrule
                 Clinical Knowledge &              34 & Spot diagnosis, joints, abdominal examination, ... & Biological Sciences \\
                 Conceptual Physics &              31 & Electromagnetism, thermodynamics, special relat... &             Physics \\
             Elementary Mathematics &              35 & Word problems, multiplication, remainders, roun... &         Mathematics \\
                       Formal Logic &              19 & Propositions, predicate logic, first-order logi... &         Mathematics \\
                       Global Facts &              15 & Extreme poverty, literacy rates, life expectanc... &              Trivia \\
                High School Biology &              35 & Cellular structure, molecular biology, ecology,... & Biological Sciences \\
              High School Chemistry &              27 &      Analytical, organic, inorganic, physical, ... & Biological Sciences \\
       High School Computer Science &              14 &        Algorithms, systems, graphs, recursion, ... &    Computer Science \\
       High School European History &              23 &   Renaissance, reformation, industrialization, ... &             History \\
              High School Geography &              27 & Population migration, rural land-use, urban pro... &              Trivia \\
High School Government and Politics &              26 & Branches of government, civil liberties, politi... &           Economics \\
         High School Macroeconomics &              35 & Economic indicators, national income, internati... &           Economics \\
         High School Microeconomics &              31 & Supply and demand, imperfect competition, marke... &           Economics \\
                High School Physics &              22 &    Kinematics, energy, torque, fluid pressure, ... &             Physics \\
             High School Psychology &              35 &     Behavior, personality, emotions, learning, ... & Biological Sciences \\
             High School Statistics &              28 & Random variables, sampling distributions, chi-s... &         Mathematics \\
           High School U.S. History &              27 & Civil War, the Great Depression, The Great Soci... &             History \\
          High School World History &              31 & Ottoman empire, economic imperialism, World War... &             History \\
                        Human Aging &              28 & Senescence, dementia, longevity, personality ch... & Biological Sciences \\
                    Human Sexuality &              17 & Pregnancy, sexual differentiation, sexual orien... & Biological Sciences \\
               Miscellaneous Topics &              35 &    Agriculture, Fermi estimation, pop culture, ... &              Trivia \\
                          Nutrition &              35 &  Metabolism, water-soluble vitamins, diabetes, ... & Biological Sciences \\
                         Philosophy &              35 & Skepticism, phronesis, skepticism, Singer’s Dro... &          Literature \\
                          Sociology &              27 & Socialization, cities and community, inequality... &          Literature \\
                U.S. Foreign Policy &              16 & Soft power, Cold War foreign policy, isolationi... &             History \\
\bottomrule
\end{tabular}

